DOMINO: A Dual-System for Multi-step Visual Language Reasoning

Visual language reasoning requires a system to extract text or numbers from information-dense images like charts or plots and perform logical or arithmetic reasoning to arrive at an answer. To tackle this task, existing work relies on either (1) an end-to-end vision-language model trained on a large amount of data, or (2) a two-stage pipeline where a captioning model converts the image into text that is further read by another large language model to deduce the answer. However, the former approach forces the model to answer a complex question with one single step, and the latter approach is prone to inaccurate or distracting information in the converted text that can confuse the language model. In this work, we propose a dual-system for multi-step multimodal reasoning, which consists of a "System-1" step for visual information extraction and a "System-2" step for deliberate reasoning. Given an input, System-2 breaks down the question into atomic sub-steps, each guiding System-1 to extract the information required for reasoning from the image. Experiments on chart and plot datasets show that our method with a pre-trained System-2 module performs competitively compared to prior work on in- and out-of-distribution data. By fine-tuning the System-2 module (LLaMA-2 70B) on only a small amount of data on multi-step reasoning, the accuracy of our method is further improved and surpasses the best fully-supervised end-to-end approach by 5.7% and a pipeline approach with FlanPaLM (540B) by 7.5% on a challenging dataset with human-authored questions.

==> sections/00_abstract_V1.tex <==
Visual-language reasoning requires a system to extract detailed information from images and perform logical or arithmetic reasoning to arrive at an answer. To tackle this task, existing work relies on either (1) %a large amount of data to train a visual language model to predict the answers directly
training a vision-language model with a large amount of data for end-to-end answer generation,
or (2) a two-stage pipeline where a captioning model converts the image into text %and then a large language model is prompted to reason over the converted text. 
that is further read by another large language model to deduce the answer.
%However, 
The former approach %forces the model to answer a complex question with one single step.
compresses a complex process of reasoning into a single step of inference, and
the latter approach %poses an unnecessary burden to the system as the converted text may contain redundant information
is prone to inaccurate or distracting visual information in the converted text that
can confuse the language model.
%while the latter poses an unnecessary burden to the system as the converted text contains redundant information which can confuse the language model \asli{Maybe too long sentence, consider splitting.}. \maryam{revised}
In this work, we propose a dual-system for multi-step multimodal reasoning, which consists of a ``System-1" step for visual information extraction and a ``System-2" step for deliberate reasoning. Given an input, System-2 breaks down the question into atomic sub-steps, each guiding System-1 to extract the information required for reasoning from the image. Experiments on chart datasets show that our method with a pre-trained System-2 module performs competitively compared to prior work on in- and out-of-distribution data. By fine-tuning the System-2 module (LLaMA-2 70B) on only a small amount of data on multi-step reasoning, the accuracy of our method is further improved and surpasses the fully-supervised approaches by $5.7\%$ and a pipeline approach with FlanPaLM (540B) by $7.5\%$ on a challenging dataset.

==> tables/intro_fig.tex <==
\setlength\intextsep{-0.4pt}
\begin{wraptable}[26]{r}{6.5cm}
%\vspace{-10pt}
\vspace{-1.5em}
\caption{\footnotesize DOMINO alternates between System-2 and System-1 to answer complex questions over charts. The chart and question are from the ChartQA dataset \citep{masry2022chartqa}.}
\small
\vspace{3pt}
\fbox{
\scalebox{0.85}
	    {
\begin{minipage}{0.5\textwidth}

\begin{singlespace*}

\raisebox{-\totalheight}{\includegraphics[width=\textwidth]{figures/introfigure.pdf}} \\\\\\

\textbf{Question}: By how many points does NET Excellent/good surpass NET Only fair/poor in Feb. 2014?\\

\noindent \hlc[mygreen]{\textbf{System-2}: Let's extract the value of NET Excellent/good in Feb. 2014.} 

 
\noindent \hspace*{\fill} \hlc[myblue]{\textbf{System-1}: The value is 54.00.} 

\noindent \hlc[mygreen]{\textbf{System-2}: Let's extract the value of NET Only fair/poor in Feb. 2014.} 

\noindent \hspace*{\fill} \hlc[myblue]{\textbf{System-1}: The value is 39.00.} 

\noindent \hlc[mygreen]{\textbf{System-2}: 54.00 surpasses 39.00 by 54.00-39.00=15.00. So the answer is 15.00.} 

\end{singlespace*}
\end{minipage}
}
}
\vspace{-5pt}
\label{introfigure}
\end{wraptable}





==> tables/num_example_ablation.tex <==
\begin{table*}[!b]
\small
\centering
\vspace{-2em}
\caption{Ablation study on how number of fine-tuning examples affects performance of the LLM. }
\label{tab:num_example_ablation}
%\vspace{3mm}
\begin{tabular}{llccccc}
\toprule
\multicolumn{1}{c}{\textbf{Evaluation Dataset}} & \multicolumn{1}{c}{\textbf{Fine-tuning Dataset}} &  \multicolumn{5}{c}{ \textbf{Number of Examples}}  \\
\cmidrule(lr){3-7} 
& & \multicolumn{1}{c}{0} & \multicolumn{1}{c}{10} & \multicolumn{1}{c}{20} & \multicolumn{1}{c}{50} & \multicolumn{1}{c}{100} \\
\midrule
PlotQA V1 &  CoT annotations & 53.1 & 46.8 & 51.2 & 52.1 & 55.0 \\
& Table reasoning annotations & 43.2 & 51.0 & 50.5 & 48.8 & 47.5 \\
\midrule
PlotQA V2 & CoT annotations & 59.0 & 57.1 & 72.2 & 77.5 & 79.6 \\
& Table reasoning annotations & 44.7 & 52.7 & 62.7 & 61.2 & 61.7 \\
\midrule
DVQA (Reasoning) &  CoT annotations & 55.2 & 56.6 & 55.8 & 55.7 & 57.5 \\
& Table reasoning annotations & 54.2 & 55.0 & 53.5 & 51.9 & 51.4 \\
\bottomrule
\end{tabular}
\end{table*}
